Modeling and Analysis of Non-unique Behaviors in Multiple Frictional Impacts

Many fundamental challenges in robotics, based in manipulation or locomotion, require making and breaking contact with the environment. To represent the complexity of frictional contact events, impulsive impact models are especially popular, as they often lead to mathematically and computationally tractable approaches. However, when two or more impacts occur simultaneously, the precise sequencing of impact forces is generally unknown, leading to the potential for multiple possible outcomes. This simultaneity is far from pathological, and occurs in many common robotics applications. In this work, we propose an approach for resolving simultaneous frictional impacts, represented as a differential inclusion. Solutions to our model, an extension to multiple contacts of Routh's method, naturally capture the set of potential post-impact velocities.We prove that solutions to the presented model must terminate. This is, to the best of our knowledge, the first such guarantee for set-valued outcomes to simultaneous frictional impacts.

==> verification.tex <==
\label{section:verification}
When $S \in \ContactSystems$ contains a large number of contacts, $S \in \NondegenerateContactSystems$ can be quite difficult to verify by hand; therefore, there is value in creating a numerical algorithm for generating certificates for this condition. To that end, we consider a slightly smaller collection of contact sets

\begin{equation}
	\NondegenerateContactSystems^* = \Braces{N \in \ContactSystems : \ZeroVector \not \in \NetForce[N]\Parentheses{\Closure\ActiveSet[N]} } \subseteq \NondegenerateContactSystems\,.
\end{equation}
For any $N \in \NondegenerateContactSystems^*$, not only is $\ZeroVector \not \in \NetForce[N]\Parentheses{\Closure\ActiveSet[N]}$, but we can find an $\epsilon > 0$ such that $\NetForce[N]\Parentheses{\Closure\ActiveSet[N]}$ is bounded at least $\epsilon$ away from $\ZeroVector$:
\begin{theorem}
	If $N \in \NondegenerateContactSystems^*$, $\exists \epsilon > 0$, $\NetForce[N]\Parentheses{\Closure\ActiveSet[N]} \cap \Ball_\epsilon = \emptyset$. 
\end{theorem}
\begin{proof}
	Suppose not. Then, for some $N \in \NondegenerateContactSystems^*$. $\exists \Sequence{\Velocity}{k}, \Sequence{\dot \Velocity}{k}$, $\Velocity_k \in \Closure\ActiveSet[N]$ and $\dot \Velocity_k \in \NetForce[N]\Parentheses{\Velocity_k}$ for all $k$ and $\dot \Velocity_k \StrongConvergence 0$. WLOG as $\dot \Velocity_k \in \NetForce[S]\Parentheses{\Direction\Velocity_k}$ for $\Velocity_k \neq \ZeroVector$, we may assume that $\Sequence{\Velocity}{k}$ is bounded. As $\Sequence{\Velocity}{k}$ and $\Sequence{\dot \Velocity}{k}$ are bounded, by dropping to a subsequence WLOG we may assume $\exists \Velocity_\infty$, $\Velocity_k \StrongConvergence \Velocity_\infty \in \Closure\ActiveSet[N]$. But then as $\NetForce[S]$ is u.s.c., $\ZeroVector \in \NetForce[S]\Parentheses{\Velocity_\infty}$ and therefore $N \not \in \NondegenerateContactSystems^*$. Contradiction!
\end{proof}
For any $\Velocity \in \Closure\ActiveSet[N], \dot \Velocity \in \NetForce[N](\Velocity)$, we have that $\dot \Velocity = \J[N]^T\Force[N]$ with $\Force[N] \in \FrictionCone[S](\Velocity)$ both bounded and bounded away from $\ZeroVector$; additionally, for any $\Velocity \not \in \Closure\ActiveSet[N]$, we have $\FrictionCone[S](\Velocity) = \{\ZeroVector\}$. Therefore, the condition $N \in \NondegenerateContactSystems^*$ is equivalent to the existence of an $\epsilon > 0$ such that
\begin{equation}
	\Force[N] \in \FrictionCone[S](\Velocity) \implies \TwoNorm{\J[N]\Force[N]}^2 - \epsilon \TwoNorm{\Force[N]}^2 \geq 0\,.\label{eq:semialgnondegenerate}
\end{equation}
We note that (\ref{eq:semialgnondegenerate}) is formatted as non-negativity of the polynomial $\TwoNorm{\J[N]\Force[N]}^2 - \epsilon \TwoNorm{\Force[N]}^2$ on a set $\FrictionCone[S](\Velocity)$ that can defined by polynomial inequalities and equalities \cite{Posa16}. Therefore, a certificate for $N \in \NondegenerateContactSystems^*$ can be generated by a sum-of-squares program that finds the maximal $\epsilon$ for which $N$ obeys (\ref{eq:semialgnondegenerate}).

